Is Cryptojacking Dead after Coinhive Shutdown?

Cryptojacking is the exploitation of victims' computer resources to mine for cryptocurrency using malicious scripts. It has become popular after 2017 when attackers started to exploit legal mining scripts, especially Coinhive scripts. Coinhive was actually a legal mining service that provided scripts and servers for in-browser mining activities. Nevertheless, over 10 million web users had been victims every month before the Coinhive shutdown that happened in Mar 2019. This paper explores the new era of the cryptojacking world after Coinhive discontinued its service. We aimed to see whether and how attackers continue cryptojacking, generate new malicious scripts, and developed new methods. We used a capable cryptojacking detector named CMTracker that proposed by Hong et al. in 2018. We automatically and manually examined 2770 websites that had been detected by CMTracker before the Coinhive shutdown. The results revealed that 99\% of sites no longer continue cryptojacking. 1\% of websites still run 8 unique mining scripts. By tracking these mining scripts, we detected 632 unique cryptojacking websites. Moreover, open-source investigations (OSINT) demonstrated that attackers still use the same methods. Therefore, we listed the typical patterns of cryptojacking. We concluded that cryptojacking is not dead after the Coinhive shutdown. It is still alive, but not as attractive as it used to be.

==> annoBib.tex <==

\section{Annotated Bibliography}

\subsection{Inadvertently Making Cyber Criminals Rich: A Comprehensive Study of Cryptojacking Campaigns at Internet Scale}

H. L. J. Bijmans, T. M. Booij, and C. Doerr, Inadvertently Making Cyber Criminals Rich: A Comprehensive Study of Cryptojacking Campaigns at Internet Scale,'' in 28th USENIX Security Symposium, 2019, pp. 1627–1644. [Online]. Available: www.usenix.org/conference/usenixsecurity19/presentation/bijman




\subsection{A first look at browser-based Cryptojacking}
Eskandari, S., Leoutsarakos, A., Mursch, T., \& Clark, J. (2018, April). A first look at browser-based Cryptojacking. In 2018 IEEE European Symposium on Security and Privacy Workshops (EuroS\&PW) (pp. 58-66). IEEE.




\subsection{End-to-end analysis of in-browser cryptojacking}
Saad, M., Khormali, A., \& Mohaisen, A. (2018). End-to-end analysis of in-browser cryptojacking. arXiv preprint arXiv:1809.02152.




\subsection{How You Get Shot in the Back: A Systematical Study about Cryptojacking in the Real World}
Hong, G., Yang, Z., Yang, S., Zhang, L., Nan, Y., Zhang, Z., ... \& Duan, H. (2018, October). How You Get Shot in the Back: A Systematical Study about Cryptojacking in the Real World. In Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security (pp. 1701-1713). ACM

This paper is a survey paper of cryptojacking. 
Cryptojacking is a threat where the client visits a website. A script code is downloaded to the client's machine and consumes the machine resources without user's consent.
They developed a behavior-based detector tool, named CMTracker, for automatically tracking Cryptocurrency Mining scripts and their related domains. 
They discovered 2,770 unique cryptojacking samples from 853,936 popular web pages, including 868 among top 100K in Alexa list.


\subsection{Web-based Cryptojacking in the Wild}
Musch, M., Wressnegger, C., Johns, M., \& Rieck, K. (2018). Web-based Cryptojacking in the Wild. arXiv preprint arXiv:1808.09474.




\subsection{An Investigation of Cryptojacking: Malware Analysis and Defense Strategies}
Marchetto, Victor. "An Investigation of Cryptojacking: Malware Analysis and Defense Strategies." Journal of Strategic Innovation and Sustainability 14, no. 1 (2019): 66-80.




\subsection{The Browsers Strike Back: Countering Cryptojacking and Parasitic Miners on the Web}
Tahir, R., Durrani, S., Ahmed, F., Saeed, H., Zaffar, F., \& Ilyas, S. (2019, April). The Browsers Strike Back: Countering Cryptojacking and Parasitic Miners on the Web. In IEEE INFOCOM 2019-IEEE Conference on Computer Communications (pp. 703-711). IEEE.




\subsection{Dynamic Analysis Framework for Cryptojacking Site Detection}
Ko, D., Jung, I., Choi, S. H., \& Choi, Y. H. (2018). Dynamic Analysis Framework for Cryptojacking Site Detection. Journal of the Korea Institute of Information Security and Cryptology, 28(4), 963-974.





\subsection{Truth in Web Mining: Measuring the Profitability and the Imposed Overheads of Cryptojacking}
Papadopoulos, P., Ilia, P., \& Markatos, E. (2019, September). Truth in Web Mining: Measuring the Profitability and the Imposed Overheads of Cryptojacking. In International Conference on Information Security (pp. 277-296). Springer, Cham.





\subsection{The Monero Project}
Getmonero.org, The Monero Project, www.getmonero.org/ Retrieved on 10/09/2019.




\subsection{In-browser mining: Coinhive and WebAssembly}
Neumann, R., \& Toro, A. (2018). In-browser mining: Coinhive and WebAssembly. Forcepoint Security Labs. Retrieved from (10/01/20019) https://www.forcepoint.com/blog/x-labs/browser-mining-coinhive-and-webassembly




\subsection{Seismic: Secure in-lined script monitors for interrupting cryptojacks}
Wang, W., Ferrell, B., Xu, X., Hamlen, K. W., \& Hao, S. (2018, September). Seismic: Secure in-lined script monitors for interrupting cryptojacks. In European Symposium on Research in Computer Security (pp. 122-142). Springer, Cham.




\subsection{Rapid: Resource and api-based detection against in-browser miners}
Rodriguez, J. D. P., \& Posegga, J. (2018, December). Rapid: Resource and api-based detection against in-browser miners. In Proceedings of the 34th Annual Computer Security Applications Conference (pp. 313-326). ACM.




\subsection{Several Cryptojacking Apps Found on Microsoft Store}
Guo,Y., Dong,T. (2019). Several Cryptojacking Apps Found on Microsoft Store. Symantec, www.symantec.com/blogs/threat-intelligence/cryptojacking-apps-microsoft-store.







